Your smartphone could act as a pulse-oximeter and as a single-lead ECG

In the post-covid19 era, every new wave of the pandemic causes an increased concern among the masses to learn more about their state of well-being. Therefore, it is the need of the hour to come up with ubiquitous, low-cost, non-invasive tools for rapid and continuous monitoring of body vitals that reflect the status of one's overall health. In this backdrop, this work proposes a deep learning approach to turn a smartphone-the popular hand-held personal gadget-into a diagnostic tool to measure/monitor the three most important body vitals, i.e., pulse rate (PR), blood oxygen saturation level (aka SpO2), and respiratory rate (RR). Furthermore, we propose another method that could extract a single-lead electrocardiograph (ECG) of the subject. The proposed methods include the following core steps: subject records a small video of his/her fingertip by placing his/her finger on the rear camera of the smartphone, and the recorded video is pre-processed to extract the filtered and/or detrended video-photoplethysmography (vPPG) signal, which is then fed to custom-built convolutional neural networks (CNN), which eventually spit-out the vitals (PR, SpO2, and RR) as well as a single-lead ECG of the subject. To be precise, the contribution of this paper is two-fold: 1) estimation of the three body vitals (PR, SpO2, RR) from the vPPG data using custom-built CNNs, vision transformer, and most importantly by CLIP model; 2) a novel discrete cosine transform+feedforward neural network-based method that translates the recorded video- PPG signal to a single-lead ECG signal. The proposed method is anticipated to find its application in several use-case scenarios, e.g., remote healthcare, mobile health, fitness, sports, etc.

==> results.tex <==
\section {Performance evaluation of vitals-Net and P2E-Net:}

\subsection{Results for Vitals-Net}

Table 4 does the performance comparison of the proposed model with the models in [34] and [35] by feeding them the two datasets, i.e., v10f-ppg and bidmc. Note that the mean and std. dev. Of the absolute error of our model is the minimum when bidmc is passed through all the three models which shows the clear superiority/optimality of our model. Note that the 1D CNN model in [34] is not designed to take 2D input that is needed for SpO2 estimation, therefore, [34] cannot do SpO2 estimation. When our dataset v10f-ppg is passed through the three models, then once again the mean and std. dev. Of the absolute error of our model is the minimum of all. 
  
\begin{table*}
\caption{\label{tab:table2_1} Absolute error performance of the DL Architecture proposed in this work, [34], [35] on the two datasets (v10f-PPG and BIDMC).
}
% \begin{large}
\begin{center}
\begin{tabular}{|c||*{12}{c|}}
\hline
~ &\multicolumn{6}{c|}{vPPG}   &   \multicolumn{6}{c|}{BIDMC}  \\\hline\hline

~ &\multicolumn{2}{c|}{HR}  & \multicolumn{2}{c|}{SpO2}  &\multicolumn{2}{c|}{RR}   & \multicolumn{2}{c|}{HR}  & \multicolumn{2}{c|}{SpO2}  &\multicolumn{2}{c|}{RR}  \\\hline

Method &$\mu$ & $\sigma$&$\mu$ & $\sigma$  & $\mu$ & \sigma & \mu &  \sigma  & \mu & \sigma & \mu & \sigma  \\\hline

Proposed     & 2.2 & 1.24  &   1.06 &0.96 &  3.15 & 0.80 & \textbf{1.46} & \textbf{0.6485} & 2.62 & 2.52 & \textbf{0.977}& \textbf{0.4769} \\\hline
\cite{reiss2019deep}      & $4.22$  & $3.76$  & -  & -&5.16 & 3.19  &  2.14& 0.925 &- &- &1.33 & 1.24  \\\hline

\cite{samavati2022efficient}	    	  &  & & &   &   &	&
2.22 &1.39  & 3.33 & 3.36 & 1.53 & 1.27 \\\hline


\end{tabular}
\end{center}
% \end{large}
\end{table*}

% /content/drive/MyDrive/Kaust_Project/packages/Plots.py
% This figure is plotted in the above file

\begin{table}
\caption{\label{tab:table3} Subject-wise Vitals Estimation Performance of Proposed DL Approach.}
% \begin{large}
\begin{center}
\begin{tabular}{|c|| c c| c  c| c c|}
\hline\hline

 Subjects&    \multicolumn{2}{c|}{HR [AE] }  & \multicolumn{2}{c|}{SpO2 [AE] }  &
 \multicolumn{2}{c|}{RR [AE]}    \\\hline\hline

& \mu   & \sigma &     \mu   & \sigma &       \mu   & \sigma       \\\hline
S1   & -  & - &     1.43 & 2.12 &     3.4  & 2.7     \\
S2   & -  & - &     1.96 & 2.62 &     3.03 & 2.6     \\
S3   & -  & - &     1.35 & 1.93 &     1.10 & 1.04    \\
S4   & -  & - &     1.29 & 0.87  &     1.44 & 1.16    \\
S5   & -  & - &     1.11 & 1.35  &     2.34 & 3.05    \\
\hline


\end{tabular}

\end{center}
% \end{large}

\end{table}

\begin{table}
\caption{\label{tab:table3} Impact of window size on the Performance of Different DL Architectures \textcolor{red}{Redundant}}
% \begin{large}
\begin{center}
\begin{tabular}{|c| c c| c  c|c| c c|}
\hline\hline

 Ws&    \multicolumn{2}{c}{HR [MAE] }  & \multicolumn{2}{c}{SpO2 [MAE] }  & Ws&
 \multicolumn{2}{c}{RR [MAE]}    \\\hline\hline

[sec]& \mu   & \sigma &     \mu   & \sigma & [sec]&       \mu   & \sigma       \\\hline
4   & 2.2  & 1.05 &     1.06 & 0.96 & 16&    2.24 & 3.09     \\
8   & 2.36 & 1.66 &     1.01 & 1.13 &24 &    2.38 & 3.31    \\
12   & 2.33  & 1.92 &    1.01 & 0.97 &\textbf{32} &    \textbf{1.59} & \textbf{2.02} \\\hline


\end{tabular}
\end{center}
% \end{large}
\end{table}

\begin{table}
\caption{\label{tab:table2}\textcolor{blue}{Values of other hyper-parameters for P2E-Vital-Net}}
% \begin{small}
\begin{center}
\begin{tabular}{|c||*{3}{c|}}
\hline

Hyper-parameters & P2E-Net& Vitals \\\hline\hline
Dataset size & $10\times10^3$&\\\hline
Test data set size & $1000$& \\\hline
Training batch size $\left(\mathcal{|F|}\right)$ & $1000$ &\\\hline
Maximum number of epochs & $\textcolor{black}{1000}$ &\\\hline
Initial learning rate & $\textcolor{black}{10^{-3}}$& \\\hline
learning rate scheduler & Exponential Decay &\\\hline
Scheduler type & Staircase &\\\hline
Lr decaying factor & exp(0.1)&\\\hline
Optimizer & Adam & \\\hline

\end{tabular}
\end{center}
 \end{table}
 
\subsection{Pulse Rate Estimation}

\begin{figure*}
% \centering
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=0.95\textwidth]{Figures/Impact_Window_size.png}
    \caption{Impact of Window Size on Vitals Estimation.}
    \label{fig:Ws_impct}
\end{subfigure}
\hfill
\hspace{0.01\textwidth}
\vspace{0.0\textwidth}
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=1\textwidth]{Figures/Channel_Impact.PNG}
    \caption{Impact of Video Channels on Vitals Estimation  .}
    \label{fig:Chnl_Impct}
\end{subfigure}


\caption{Optimal video channels and Window Size for Vitals estimation.}
\label{fig:figures}
\end{figure*}






\subsection{SpO2 Estimation}

\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=1.2\textwidth]{Figures/RR_test.png}
        \caption{Error in RR Estimation}
        \centering
        \label{fig:RR_error}
    \end{subfigure}
    % \hfill
    
    \hspace{0.03\textwidth}
    \vspace{0.0\textwidth}
    
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[width=1.2\textwidth]{Figures/SpO2_test.png}
        \caption{Error in SpO2 Estimation}
        \centering
        \label{fig:SpO2_error}
    \end{subfigure}
    \label{fig:SpO2_Loss}
    \caption{Losses of Vitals Estimation}
\end{figure}



% \begin{figure}
% \centering
% \includegraphics[width=3.6in]{Figures/SpO2_loss.png}
% \caption{Losses of SpO2 Estimation}
% \centering
% \label{fig:SpO2_Loss}
% \end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=3.6in]{Figures/RR_loss.png}
% \caption{Losses of RR Estimation}
% \centering
% \label{fig:RR_Loss}
% \end{figure}


% \begin{table}
% \caption{\label{tab:table2_1} Impact of video RGB channels on the performance\textcolor{red}{Redundant}.}
% \begin{small}
% \begin{center}
% \begin{tabular}{|c||*{6}{c|}}
% \hline

% Subjects &HR [mean] & HR [std]  & SpO2 [mean] & SpO2 [std] & RR [mean]   & RR [std]  \\\hline\hline

% Red      & 2.2  & 1.05   & 1.07 & 1.08 &  1.71 &   1.74     \\\hline
% Green    & 2.2  & 2.44   & 1.05 & 0.94 &  2.24  &  2.22       \\\hline
% Blue     & 3.5  & 2.07 ` & 1.31 & 2.46 &  1.86 & 1.82  \\\hline


% \end{tabular}
% \end{center}
% \end{small}
% \end{table}



\subsection{Results for P2E-Net}
%\subsection{P2E-Net: Experimental Results}
Fig. \ref{fig:ppg_ref_syn_ecg} plots the PPG signal, the reference ECG signal (acquired by MAX86150 module), and the synthetic ECG signal (outputed by the P2E-Net) in parallel, for 4 different subjects. We notice that the morphology of the synthetic ECG signal is very similar to the morphology of the reference ECG signal as both ECG waveforms observe the QRS complex and T waves. However, the R peaks of synthetic ECG signal have a different amplitude than their counterparts in the reference ECG signal. 

\begin{figure*}
\centering
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1.2\textwidth]{Figures/Rcnstctd_ecg6.jpg}
    % \caption{Firts subfigure.}
    % \label{fig:first}
\end{subfigure}
% \hfill
\hspace{0.03\textwidth}
\vspace{0.0\textwidth}
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1.2\textwidth]{Figures/Rcnstctd_ecg33.jpg}
    % \caption{Second subfigure.}
    % \label{fig:second}
\end{subfigure}
\hspace{0.03\textwidth}
\vspace{0.00\textwidth}
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1.2\textwidth]{Figures/Rcnstctd_ecg47.jpg}
    % \caption{Third subfigure.}
    \label{fig:third}
\end{subfigure}
\hspace{0.03\textwidth}
\vspace{0.00\textwidth}
\begin{subfigure}{0.4\textwidth}
    \includegraphics[width=1.2\textwidth]{Figures/Rcnstctd_ecg36.jpg}
    % \caption{Third subfigure.}
    \label{fig:third}
\end{subfigure}
        
\caption{Performance of P2E-Net}
\label{fig:ppg_ref_syn_ecg}
\end{figure*}

{\it Testing of proposed P2E-Net via an atrial fibrillation detector:} The clinical significance of single-lead ECG lies in the fact that it could detect atrial fibrillation (i.e., abnormal/irregular heartbeat). Let us label a sample of normal sinus rhythm (i.e., regular heartbeat) as "normal", and a sample with atrial fibrillation as "abnormal". In this backdrop, we did two controlled experiments (first using v10f-PPG dataset, second using BIDMC dataset) to assess the credibility of the proposed P2E-Net framework. 1) We considered 7 normal examples from v10f-PPG dataset and passed their video-PPG data component through the P2E-Net which returned us the 7 synthetic ECG waveforms. We then passed the 7 synthetic ECGs through an atrial fibrillation detector (a binary ML classifier) which correctly classified all of them as normal. 2) We considered 41 samples (37 normal samples, 4 abnormal samples) from BIDMC dataset and passed their PPG data component through the P2E-Net which returned us the 41 synthetic ECG waveforms. We then passed the 41 synthetic ECGs through the atrial fibrillation detector which correctly classified 34 of 37 samples as normal, and 4 of 4 samples as abnormal. This exercise demonstrates that the proposed P2E-Net method indeeds synthesizes accurate ECG waveforms. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
% \centering
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=1\textwidth]{Figures/Impact_of_DCT_coeff.png}
    \caption{Impact of number of DCT Coefficients.}
    \label{fig:impct_dct_coeff}
\end{subfigure}
\hfill
\hspace{0.01\textwidth}
\vspace{0.0\textwidth}
\begin{subfigure}{0.5\textwidth}
    \includegraphics[width=1\textwidth]{Figures/Impct_Num_crdc_cycl.png}
    \caption{Impact of Number of Cardiac Cycles.}
    \label{fig:Chnl_Impct}
\end{subfigure}


\caption{Optimal video channels and Window Size for Vitals estimation.}
\label{fig:figures}
\end{figure*}



% \begin{figure}
% \centering
% \includegraphics[width=3.5in]{Figures/Cardiac_cycles_impact.png}
% \caption{Impact of Number of Cardiac Cycles on reconstructed 
% ECG}
% \centering
% \label{fig:SpO2_error}

% \end{figure}




% \begin{table*}%[!ht]
%     \caption{\label{tab:table2_1} Impact of number of cardiac cycles and/or number of ECG DCT coeff.}
%     \begin{large}
%     \begin{center}
%     \begin{tabular}{|l|l|l|l|l|l|l|}
%     \hline
%         ~ & MAE & ~ & Pcorr & ~ & Frec. dist & ~ \\ \hline
%         Card. Cyc. & \mu & \sigma & \mu & \sigma & \mu & \sigma \\ \hline
%         1 & 0.075 & 0.022 & 0.828 & 0.097 & 0.447 & 0.071 \\ \hline
%         2 & 0.074 & 0.020 & 0.728 & 0.178 & 0.444 & 0.102 \\ \hline
%         3 & 0.078 & 0.020 & 0.675 & 0.207 & 0.435 & 0.085 \\ \hline
%         DCT Coeff. & \mu & \sigma & \mu & \sigma & \mu & \sigma \\ \hline
%         100 & 0.075 & 0.022 & 0.828 & 0.097 & 0.447 & 0.071 \\ \hline
%         120 & 0.064 & 0.016 & 0.826 & 0.102 & 0.244 & 0.120 \\ \hline
%         150 & 0.062 & 0.011 & 0.823 & 0.106 & 0.214 & 0.114 \\ \hline
        
%     \end{tabular}
%     \end{center}
%     \end{large}
% \end{table*}

%\begin{figure}
%\centering
%\begin{subfigure}{0.45\textwidth}
%    \includegraphics[width=0.9\textwidth]{Figures/confusion_mat.png}
    % \caption{Channel Impact on HR estimation.}
    % \label{fig:first}
%\end{subfigure}
% \hfill
% \hspace{0.04\textwidth}
%\vspace{0.0\textwidth}
%\caption{Confusion Matrix 1 representing 100 percent.}
%\label{fig:figures}
%\end{figure}


\begin{table*}
\caption{\label{tab:table2_1} Performance of P2E-Net. Mean and Std. of 5 subjects' peaks and Valleys.
}
% \begin{large}
\begin{center}
\begin{tabular}{|c||*{10}{c|}}
\hline
~ &\multicolumn{10}{c|}{vPPG}       \\\hline\hline

Method &\multicolumn{2}{c|}{P-Peaks}  & \multicolumn{2}{c|}{Q-Valleys}  &\multicolumn{2}{c|}{R-Peaks}  & \multicolumn{2}{c|}{S-Valleys} & \multicolumn{2}{c|}{T-Peaks}   \\\hline

~ & MMAE & MSAE &MMAE & MSAE  &MMAE& MSAE & MMAE & MSAE &MMAE & MSAE   \\\hline

DCT+Ridge    & $0.0487$ & $0.01996$   & 0.05722 & 0.0243 &  0.0883 & 0.0419 &  0.0850
 &   0.0291    &0.1125 & 0.0319\\\hline
 
DCT+NN      & \textbf{0.0418}&	0.0177&	0.0612&	0.0177&	0.059&	0.0381&	0.09516&	0.0303&	0.1044&	0.0275\\\hline
% ~ &\multicolumn{10}{c|}{BMDIC}       \\\hline\hline

\end{tabular}
\end{center}
\end{table*}

{\it Machine specifications.} 
Central Processing Unit (CPU) used was Intel Core i7-4770 @ 3.40 GHz. Random Access Memory (RAM) size was $4$ GB. The operating system was $64$bit Microsoft Windows.

==> section2.tex <==
\section{Contribution 1: v10f-PPG dataset}

Before we outline the details of our v10f-PPG dataset, it is imperative to provide the reader with a systematic and brief review of the relevant existing public datasets on video-PPG (as well as their limitations)\footnote{Note that there are PPG datasets constructed using commercial pulse oximeters, e.g., MIMIC-III dataset \cite{johnson2016mimic}, \cite{liang2018new}, video-PPG datasets based upon traditional cameras \cite{mcduff} (before the advent of smartphones), and video-PPG datasets that utilize PPG signals for biometrics/authentication purposes, e.g., biosec1 dataset \cite{8411233}. But since this work primarily focuses on video-PPG datasets acquired using smartphones for vitals estimation, discussion of such datasets (and the corresponding works) are out of scope of this work.}.




\subsection{Existing video-PPG datasets}

%The state-of-art deep learning-based vital estimation approaches mainly rely remote video PPGs either taken from wrists, forehead or face.    

%\textcolor{orange}{Note: This dataset is not public. So, no need to mention it here. Adding in Table.}
%\textcolor{orange}{iPPG \cite{5963704} is one of the earliest data sets which is publicly available. This data set was recorded with Motorola Droid camera. The iPPG video was recorded from the Palmer side of the index finger of the left hand under flashlight-on conditions. Moreover, the ECG signal was also recorded simultaneously to get the HR and RR ground truths. Furthermore, the ground truth of SpO2 was recorded by a commercial pulse oximeter (Radical SET$^{TM}$, Masimo). RR ground truth was taken using a Respiratory belt worn on the chest.}

\textit{1) BUT-PPG dataset \cite{nemcova2021brno}}:   
This dataset contains 48 simultaneous records of video-PPG data and single-lead ECG data of 12 healthy subjects (6 males, 6 females), 21 to 61 years old. Each video of the index finger of the subject was recorded for a duration of 10 seconds, using a Xiaomi MI9 smartphone at a frame rate of 30Hz. The single-lead ECG data was recorded using a Bittium Faros 360 device at sampling rate of 1000 Hz, and was manually annotated by an expert. Eventually, \cite{nemcova2021brno} utilized their dataset to estimate the HR.

\textit{2) Welltory dataset \cite{neshitov2021wavelet}}:  
This dataset contains 21 records of video-PPG data of 13 healthy subjects, 25 to 35 years old. Each video of the index finger of the subject was recorded for a duration between 1-2 minutes, using Welltory android app. The R-peak to R-peak (RR) intervals were recorded using a Polar H10 ECG chest strap, and were manually examined by an expert. Eventually, \cite{neshitov2021wavelet} utilized their dataset to estimate the HR and HRV.

\textit{3) MTHS dataset \cite{08989}}:  
This dataset contains 65 recording of video-PPG data along with corresponding HR and SpO2 labels, of 62 patients (35 males, 27 females). Each video of the index finger of the subject was recorded using an iPhone 5s smartphone at a frame rate of 30Hz. The ground truth/labels were obtained using a pulse oximter (M70) at a sampling rate of 1 Hz. Eventually, \cite{08989} utilized their dataset to estimate the HR and SpO2.

{\it Limitations of existing video-PPG datasets:} We identified many limitations/shortcomings of the aforementioned video-PPG datasets, some of them are as follows. The BUT-PPG dataset provides labels for HR only, while the Welltory dataset provides labels for HR and HRV only. Moreover, the small size of BUT-PPG and Welltory datasets renders them infeasible for state-of-the-art but data-hungry deep learning methods. The MTHS dataset though contains sufficient examples (enough to train a neural network) but provides labels for HR and SpO2 only. More importantly, the need for a new and large dataset on video-PPG stems from the fact that the generalization capability, accuracy, and robustness of any deep learning algorithm for vitals estimation could only be tested if a handful of video-PPG datasets are publicly available.  

\subsection{Our dataset: The v10f-PPG dataset}
The limitations of the existing video-PPG datasets (e.g., small number of training examples, lack of raw data and labels for RR and single-lead ECG, as needed by our study) prompted us to run an extensive campaign for video-PPG data collection of our own. Thus, we subsequently compiled a large new dataset which we named as v10f-PPG dataset. The data collection campaign was approved by the ethical institutional review board (EIRB) of ITU, Lahore, Pakistan, and all the subjects voluntarily participated in this data collection activity. Next, we discuss all the relevant details of the v10f-PPG dataset, e.g., participants, data characteristics, data acquisition setup, ground truth acquisition, synchronization of PPG and ECG waveforms etc.  

{\it Participants:}
A total of 50 healthy subjects with no history of any cardiac or respiratory disease participated in this data collection campaign, out of which 10 were females and 40 were males. The volunteers/participants were either employees or students at our institute, aged 16-36 years. 

{\it Data characteristics:} For each subject, we recorded the minute-long video-PPG data (the raw data) of all the ten fingers of the two hands. Thus, we collected 10 minutes of video-PPG data from each subject, and consequently, a total of 500 minutes of video-PPG data from all the 50 subjects. For ground truth/labels for supervised learning later, we simultaneously recorded the three body vitals (PR, SpO2, RR) and single-lead ECG of each subject. We also collected following additional features/meta-data for each subject: height, weight, age, and gender.


\begin{table*}
\caption{\label{tab:table2_1} \textcolor{red}{Comparison of datasets: Labels Frequency.} }
% \begin{large}
\begin{center}
\begin{tabular}{|c||*{10}{c|}}
\hline

PR [bpm] & \multicolumn{3}{c|}{ counts } & SpO2 [\%] & \multicolumn{2}{c|}{ counts } & RR [rpm] & \multicolumn{2}{c|}{ counts } \\\hline\hline

 Range     & v10f-PPG        & Welltory & BIDMC & Range & v10f-PPG & BIDMC & Range & v10f-PPG & BIDMC \\\hline

0-40   &  0            & 0   & 10 &00-90  &108   &  473  &0-5& 188\times 3&  175  \\\hline
40-60  & \textbf{64}  & 52  & 323&90-92   &0    &  468    &5-10&601 \times 3& 340    \\\hline
60-80  & \textbf{3899} & 575&5102 &92-94  &55    & 3413    &10-15 & 1741 \times 3&3814   \\\hline
80-100 & \textbf{4319} & 126&14150 &94-96  &1201  & 3994    &15-20 &799 \times 3 &16146   \\\hline
100-120& \textbf{52}   & 0  &3116 &96-98  &5706  & 7342   &20-25& 426 \times 3& 2802  \\\hline
120-140& \textbf{86}  & 0   &   905
 &98-100 &1581  & 7916   &25-40&237\times 3&  151 \\\hline

\end{tabular}
\end{center}
% \end{large}
\end{table*}

{\it Equipment used for data acquisition:}
The video-PPG data of the finger tips of the subjects was recorded using the rear camera of Huawei ShotX smartphone. The ground truth/labels for the three vitals (PR, SpO2, RR) of the subjects were collected using Masimo MightySat and Beurer P080 pulse-oximeters. The reference single-lead ECG of the subjects was recorded using the Max86150 single-lead ECG module.

{\it Data acquisition setup:}
Fig. 2 (a) shows the experimental setup to collect the labeled data for the vitals estimation problem, while Fig. 2 (b) shows the experimental setup to collect the labeled data for PPG2ECG translation problem. Some more elaborate details of the data acquisition process are as follows. Before the beginning of data collection, the subject was asked to sit on the chair in a comfortable way and rest his/her arm on the empty table. The heights of table and chair were adjusted in such a way that the arms and heart remain at almost the same level of height. Then, the periodic change of color of fingertip due to blood volume change due to rhythmic cardiac activity was recorded as a video using rear camera of Huawei ShotX smartphone. For the experiment of Fig. 2 (a), a commercial transmittance type pulse-oximeter (Beurer PO80) and another pulse-oximeter (Masimo MightySat) were used to simultaneously record the ground truth of the three vitals (PR, SpO2, RR). For the experiment of Fig. 2 (b), the Max86150 single-lead ECG module was used to simultaneously record the reference single-lead ECG of the subjects. A minute-long video was recorded from each finger of both left and right hand. Subjects were instructed to put on the pulse-oximeter on the index finger of right hand while recording the video-PPG data from each fingertip of left hand, and vice versa. For recording of video-PPG data, subjects were instructed to place the Palmer side of each finger one by one on the camera lens of smartphone with the flash light turned on. They were also instructed to avoid pressing the camera lens with additional force. During the data acquisition activity, subjects were allowed to talk. The video-PPG data was recorded at a frame rate of 30 frames per second, with a frame resolution of 1024x480 pixels. Here, it is worth mentioning that the video start and stop times were also noted manually, and this information was used later for the synchronization of PPG and ECG waveforms. The ground truths were recorded using the pulse oximeter at a sampling rate of 0.5 Hz. 

{\it Synchronization of raw video-PPG data with labels:}
 The video-PPG data for each fingertip of each subject was synchronized with its labels/ground truths manually, and with the great care. 
 
{\it Data inclusion-exclusion algorithm:} To ensure that only high-quality samples are collected for the v10f-PPG dataset, a data inclusion-exclusion algorithm similar to the one described in \cite{liang2018new} was utilized, and is briefly described as follows. For every sample, do the following. If the ground truth(s) are corrupted, then discard the sample (data integrity screening). If the recorded video file is corrupted, then discard the sample (video quality screening). If the quality of the PPG signal extracted from video-PPG signal is low, discard the sample (PPG signal quality screening). Otherwise, add the sample to the dataset. A direct consequence of this algorithm is that for some subjects, some fingertip videos were eventually discarded to enforce quality control check. 

%\begin{figure}
%\centering
%\includegraphics[width=3.3in]{Figures/Age Statics.png}
%\caption{Age Statistics [Histogram of Age Group].}
%\centering
%\label{fig:age_stats}
%\end{figure}

\begin{table*}
\caption{\label{tab:table2_1} \textcolor{red}{Comparison of datasets: subject-wise Vitals Ground Truth Values Details.} }
% \begin{large}
\begin{center}
\begin{tabular}{|c||*{14}{c|}}
\hline
~ &\multicolumn{6}{c|}{v10f-PPG}   & \multicolumn{2}{c|}{Welltory}   & \multicolumn{6}{c|}{BIDMC}  \\\hline\hline

~ &\multicolumn{2}{c|}{PR}  & \multicolumn{2}{c|}{SpO2}  &\multicolumn{2}{c|}{RR}  & \multicolumn{2}{c|}{PR} & \multicolumn{2}{c|}{PR}  & \multicolumn{2}{c|}{SpO2}  &\multicolumn{2}{c|}{RR}  \\\hline

Subjects & $\mu$ & $\sigma$&$\mu$ & $\sigma$  & $\mu$ & \sigma & \mu & \sigma &\mu & \sigma  & \mu & \sigma & \mu & \sigma  \\\hline

S1      & 78.93  & 7.54   & 95.12 & 7.47&11.87&2.44 &  50.87 &   0.59     &81&0.48&99&0&21.42&1.23\\\hline
S2      & 85.35  & 4.87   & 98.35 & 0.48&10.72& 4.31&  83.0  &  2.41       &90&0.38&95&0.017&15.35&0.91\\\hline
S3      & 77.25  & 6.57  & 96.44 & 1.23&16.55&0.32 &  82.25 & 2.72  &100&0.67&93&0&17.64&0.71\\\hline
S4	    & 117.0  & 2.05	  & 98.56 &0.51&12.54& 4.71 &  74.50 &	3.72
&77&0.64&97&0.66&16.67& 0.74\\\hline
S5	    & 103.5  & 4.68	  & 97.6 &0.53&10.71& 4.76 &  73.12 &	2.51 &81&1.35&98&1.29&11.47&1.64
\\\hline

\end{tabular}
\end{center}
% \end{large}
\end{table*}

\subsection{Benchmark dataset: The BIDMC dataset}
As we mentioned earlier in this section, one could learn more about the generalization capability, accuracy, and robustness of his/her proposed deep learning algorithm by testing it on other datasets (with unseen data with potentially different distribution). Therefore, this work utilizes the well-known BIDMC dataset \cite{pimentel2016toward} (in addition to the v10f-PPG dataset) for the training and performance evaluation of proposed method for vitals estimation. Some most pertinent details of the BIDMC dataset are as follows. The BIDMC dataset contains 54 sessions (each of duration eight minutes) of simultaneously recorded PPG and ECG signals, along with the ground truth values (i.e., the vitals). The PPG and ECG signals are recorded at a sampling frequency of 125 Hz, whereas the ground truth values of HR, SpO2 and RR are recorded at a sampling rate of 1 Hz. Note that the PPG signals in this dataset were acquired from the fingertip of patients using the clinical pulse oximeter. Finally, the single-lead ECG signal collected in this dataset is the Lead-II acquired using the standdard 12-lead ECG.  
